On Disentangling Spoof Trace for Generic Face Anti-Spoofing

Prior studies show that the key to face anti-spoofing lies in the subtle image pattern, termed "spoof trace", e.g., color distortion, 3D mask edge, Moire pattern, and many others. Designing a generic anti-spoofing model to estimate those spoof traces can improve not only the generalization of the spoof detection, but also the interpretability of the model's decision. Yet, this is a challenging task due to the diversity of spoof types and the lack of ground truth in spoof traces. This work designs a novel adversarial learning framework to disentangle the spoof traces from input faces as a hierarchical combination of patterns at multiple scales. With the disentangled spoof traces, we unveil the live counterpart of the original spoof face, and further synthesize realistic new spoof faces after a proper geometric correction. Our method demonstrates superior spoof detection performance on both seen and unseen spoof scenarios while providing visually convincing estimation of spoof traces. Code is available at https://github.com/yaojieliu/ECCV20-STDN.

==> figures/table-siwm-p1.tex <==
\begin{table}[t]
\caption{\small The evaluation on SiW-M Protocol I: known spoof detection.}
\centering
	\resizebox{0.8\textwidth}{!}{
	\begin{tabular}{llllllllllllllllll}
	\multicolumn{17}{c}{} \\ \toprule
	\multirow{2}{*}{Metrics(\%)} &\multirow{2}{*}{Replay}& \multirow{2}{*}{Print} & \multicolumn{5}{c}{3D Mask}  && \multicolumn{3}{c}{Makeup}  &&  \multicolumn{3}{c}{Partial Attacks} & \multirow{2}{*}{Overall}\\ 
	\cline{4-8} \cline{10-12} \cline{14-16}
	& & & Half & Silic. & Trans. & Paper & Manne. && Ob. & Im. & Cos. && Funny. & Papergls. & Paper &\\ \hline
	%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
	\iffalse
    APCER
        &$0.3$& $0.1$ & $0.0$ & $12.0$ & $0.0$ & $0.7$ & $3.4$ & $0.0$ & $0.0$ & $42.8$ & $2.1$ & $1.4$ & $0$ & $2.1$ \\
    BPCER
        &\multicolumn{14}{|c}{$6.1$}  \\ \hline
    \fi
    %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% ACER %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
	\multicolumn{17}{c}{ACER(\%)} \\ \hline
    Auxiliary\cite{liu-auxiliary-fas}
        &$5.1$& $5.0$ & $5.0$ & $10.2$ & $5.0$ & $9.8$ & $6.3$ && $19.6$ & $5.0$ & $26.5$ && $5.5$ & $5.2$ & $5.0$ & $6.3$ \\
    Ours
        &$\textbf{3.2}$& $\textbf{3.1}$ & $\textbf{3.0}$ & $\textbf{9.0}$ & $\textbf{3.0}$ & $\textbf{3.4}$ & $\textbf{4.7}$ && $\textbf{3.0}$ & $\textbf{3.0}$ & $\textbf{24.5}$ && $\textbf{4.1}$ & $\textbf{3.7}$ & $\textbf{3.0}$ & $\textbf{4.1}$ \\ \hline
    %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% EER %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
	\multicolumn{17}{c}{EER(\%)} \\ \hline
    Auxiliary\cite{liu-auxiliary-fas}
        &$4.7$& $0.0$ & $1.6$ & $10.5$ & $4.6$ & $10.0$ & $6.4$ && $12.7$ & $0.0$ & $19.6$ && $7.2$ & $7.5$ & $0.0$ & $6.6$ \\
    Ours
        &$\textbf{2.1}$& $\textbf{2.2}$ & $\textbf{0.0}$ & $\textbf{7.2}$ & $\textbf{0.1}$ & $\textbf{3.9}$ & $\textbf{4.8}$ && $\textbf{0.0}$ & $\textbf{0.0}$ & $\textbf{19.6}$ && $\textbf{5.3}$ & $\textbf{5.4}$ & $\textbf{0.0}$ & $\textbf{4.8}$ \\ \hline
    \multicolumn{17}{c}{TDR@FDR=$0.5$(\%)} \\ \hline
    Ours
        &$90.1$& $76.1$ & $80.7$ & $71.5$ & $62.3$ & $74.4$ & $85.0$ && $100.0$ & $100.0$ & $33.8$ && $49.6$ & $30.6$ & $97.7$ & $70.4$ \\ \bottomrule
	\end{tabular}
\label{tab:siwm_p1}} 
\figvspace
\end{table}
